Three-boson stability for boosted interactions towards the zero-range limit

We study the three-boson bound-state mass and wave functions for ground and excited states within the three-body relativistic framework with Kamada and Gl\"ocke boosted potentials in the limit of a zero-range interaction. We adopt a nonrelativistic short-range separable potential, with Yamaguchi and Gaussian form factors, and drive them towards the zero-range limit by letting the form factors' momentum scales go to large values while keeping the two-body binding fixed. We show that the three-boson relativistic masses and wave functions are model-independent towards the zero-range limit, and the Thomas collapse is avoided, while the nonrelativistic limit kept the Efimov effect. Furthermore, the stability in the zero-range limit is a result of the reduction of boosted potential with the increase of the virtual pair center of mass momentum within the three-boson system. Finally, we compare the present results with Light-Front and Euclidean calculations.

==> Referencesbib <==

@article{PhysRevA.85.023610,
  title = {Binding and structure of tetramers in the scaling limit},
  author = {Hadizadeh, M. R. and Yamashita, M. T. and Tomio, Lauro and Delfino, A. and Frederico, T.},
  journal = {Phys. Rev. A},
  volume = {85},
  issue = {2},
  pages = {023610},
  numpages = {22},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.85.023610}
}


@article{PhysRevC.90.054002,
  title = {Relativistic three-body bound state in a 3D formulation},
  author = {Hadizadeh, M. R. and Elster, Ch. and Polyzou, W. N.},
  journal = {Phys. Rev. C},
  volume = {90},
  issue = {5},
  pages = {054002},
  numpages = {12},
  year = {2014},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.90.054002}
}

@article{wang2018colloquium,
  title={Colloquium: Excitons in atomically thin transition metal dichalcogenides},
  author={Wang, Gang and Chernikov, Alexey and Glazov, Mikhail M and Heinz, Tony F and Marie, Xavier and Amand, Thierry and Urbaszek, Bernhard},
  journal={Reviews of Modern Physics},
  volume={90},
  number={2},
  pages={021001},
  year={2018},
  publisher={APS},
  doi={10.1103/RevModPhys.90.021001}
}

@article{berkelbach2013theory,
  title={Theory of neutral and charged excitons in monolayer transition metal dichalcogenides},
  author={Berkelbach, Timothy C and Hybertsen, Mark S and Reichman, David R},
  journal={Physical Review B},
  volume={88},
  number={4},
  pages={045318},
  year={2013},
  publisher={APS},
  doi={10.1103/PhysRevB.88.045318}
}

@article{kormanyos2015k,
  title={k{\textperiodcentered} p theory for two-dimensional transition metal dichalcogenide semiconductors},
  author={Korm{\'a}nyos, Andor and Burkard, Guido and Gmitra, Martin and Fabian, Jaroslav and Z{\'o}lyomi, Viktor and Drummond, Neil D and Fal’ko, Vladimir},
  journal={2D Materials},
  volume={2},
  number={2},
  pages={022001},
  year={2015},
  publisher={IOP Publishing},
  doi={10.1088/2053-1583/2/4/049501}
}

@article{chaves2017excitonic,
  title={Excitonic effects in the optical properties of 2D materials: An equation of motion approach},
  author={Chaves, AJ and Ribeiro, RM and Frederico, T and Peres, NMR},
  journal={2D Materials},
  volume={4},
  number={2},
  pages={025086},
  year={2017},
  publisher={IOP Publishing},
  doi={10.1088/2053-1583/aa6b72}
}

@article{zhang2017two,
  title={Two dimensional hexagonal boron nitride (2D-hBN): synthesis, properties and applications},
  author={Zhang, Kailiang and Feng, Yulin and Wang, Fang and Yang, Zhengchun and Wang, John},
  journal={Journal of Materials Chemistry C},
  volume={5},
  number={46},
  pages={11992--12022},
  year={2017},
  publisher={Royal Society of Chemistry},
  doi={10.1039/C7TC04300G}
}

@article{ferreira2019excitons,
  title={Excitons in hexagonal boron nitride single-layer: a new platform for polaritonics in the ultraviolet},
  author={Ferreira, F and Chaves, AJ and Peres, NMR and Ribeiro, RM},
  journal={JOSA B},
  volume={36},
  number={3},
  pages={674--683},
  year={2019},
  publisher={Optical Society of America},
  doi={10.1364/JOSAB.36.000674}
}

@article{KAMADA2007119,
title = {Realistic two-nucleon potentials for the relativistic two-nucleon Schrödinger equation},
author = {H. Kamada and W. Glöckle},
journal = {Physics Letters B},
volume = {655},
number = {3},
pages = {119-125},
year = {2007},
issn = {0370-2693},
doi = {10.1016/j.physletb.2007.07.071}
}

@article{hadizadeh2017calculation,
Author = {Hadizadeh, M. R. and Radin, M. },
Journal = {The European Physical Journal A},
Number = {2},
Pages = {18},
Publisher = {Springer},
Title = {Calculation of relativistic nucleon-nucleon potentials in three dimensions},
Volume = {53},
Year = {2017},
doi = {10.1140/epja/i2017-12209-6}
}
	
@article{hadizadeh2020three,
  title={A three-dimensional momentum-space calculation of three-body bound state in a relativistic Faddeev scheme},
  author={Hadizadeh, M. R. and Radin, M. and Mohseni, K.},
  journal={Scientific Reports},
  volume={10},
  number={1949},
  year={2020},
  publisher={Nature Publishing Group},
  doi = {10.1038/s41598-020-58577-4}
}	

@article{hadizadeh2021nnrelativistic,
  title={Relativistic nucleon-nucleon potentials in a spin-dependent three-dimensional approach},
  author={Hadizadeh, M. R. and Radin, M. and Nazari, M.},
 journal={Scientific Reports},
  volume={11},
  number={17550},
  year={2021},
  publisher={Nature Publishing Group},
  doi = {10.1038/s41598-021-96924-1}
}

@article{Frederico:1992np,
    author = "Frederico, T.",
    title = "{Null plane model of three bosons with zero range interaction}",
    doi = "10.1016/0370-2693(92)90661-M",
    journal = "Phys. Lett. B",
    volume = "282",
    pages = "409--414",
    year = "1992"
}

@article{Karmanov:2003qk,
    author = "Karmanov, V. A. and Carbonell, J.",
    title = "{Critical stability of three body relativistic bound states with zero range interaction}",
    eprint = "nucl-th/0310064",
    archivePrefix = "arXiv",
    doi = "10.1007/s00601-004-0027-5",
    journal = "Few Body Syst.",
    volume = "34",
    pages = "85--90",
    year = "2004"
}

@article{Carbonell:2002qs,
    author = "Carbonell, J. and Karmanov, V. A.",
    title = "{Three boson relativistic bound states with zero range interaction}",
    eprint = "nucl-th/0207073",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevC.67.037001",
    journal = "Phys. Rev. C",
    volume = "67",
    pages = "037001",
    year = "2003"
}

@article{Karmanov:2009bhn,
    author = "Karmanov, V. A. and Maris, P.",
    title = "{Manifestation of three-body forces in three-body Bethe-Salpeter and light-front equations}",
    eprint = "0811.1100",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/s00601-009-0054-3",
    journal = "Few Body Syst.",
    volume = "46",
    pages = "95--113",
    year = "2009"
}

@article{YDREFORS2017131,
title = {Three-body bound states with zero-range interaction in the Bethe–Salpeter approach},
author = {E. Ydrefors and J.H. {Alvarenga Nogueira} and V. Gigante and T. Frederico and V.A. Karmanov},
journal = {Physics Letters B},
volume = {770},
pages = {131-137},
year = {2017},
issn = {0370-2693},
doi = {10.1016/j.physletb.2017.04.035}
}

@article{Ydrefors:2019jvu,
    author = "Ydrefors, E. and Alvarenga Nogueira, J. H. and Karmanov, V. A. and Frederico, T.",
    title = "{Solving the three-body bound-state Bethe-Salpeter equation in Minkowski space}",
    eprint = "1903.01741",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.physletb.2019.02.046",
    journal = "Phys. Lett. B",
    volume = "791",
    pages = "276--280",
    year = "2019"
}

@article{Ydrefors:2020duk,
    author = "Ydrefors, E. and Alvarenga Nogueira, J. H. and Karmanov, V. A. and Frederico, T.",
    title = "{Three-boson bound states in Minkowski space with contact interactions}",
    eprint = "2005.07943",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.101.096018",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "9",
    pages = "096018",
    year = "2020"
}


@article{elster1999three,
  title={Three-body bound-state calculations without angular-momentum decomposition},
  author={Elster, Ch. and Schadow, W. and Nogga, A. and Gl{\"o}ckle, W.},
  journal={Few-Body Systems},
  volume={27},
  number={2},
  pages={83--105},
  year={1999},
  publisher={Springer},
  doi ={10.1007/s006010050124}
}

@article{PhysRev.95.1628,
  title = {Two-Nucleon Problem When the Potential Is Nonlocal but Separable. I},
  author = {Yamaguchi, Y.},
  journal = {Phys. Rev.},
  volume = {95},
  issue = {6},
  pages = {1628--1634},
  numpages = {0},
  year = {1954},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.95.1628}
}

@article{platter2004four,
title={Four-boson system with short-range interactions},
author={Platter, Lucas and Hammer,H-W and Mei{\ss}ner, Ulf-G},
journal={Physical Review A},
volume={70},
number={5},
pages={052101},
year={2004},
publisher={APS},
doi = {10.1103/PhysRevA.70.052101}
}

@article{deltuva2011universality,
title={Universality in four-body scattering},
author={Deltuva, A. and Lazauskas, R. and Platter, L.},
journal={Few-Body Systems},
volume={51},
number={2},
pages={235--247},
year={2011},
publisher={Springer},
doi = {10.1007/s00601-011-0227-8}
}

@article{Coester1975,
title={Relativistic effects in phenomenological nucleon-nucleon potentials and nuclear matter},
author={Coester, F, and Pieper, S. C. and Serduke, F. J. D.},
journal={Phys. Rev. C},
volume={11},
number={1},
pages={1},
year={1975},
publisher={APS},
doi={10.1103/PhysRevC.11.1}
}

@article{Keister2006,
  title={Quantitative relativistic effects in the three-nucleon problem},
  author={Keister, B. D., and Polyzou, W. N.},
  journal={Phys. Rev. C},
  volume={73},
  number={1},
  pages={014005},
  year={2006},
  publisher={APS},
  doi={10.1103/PhysRevC.73.014005}
}

@book{Gattringer:2010zz,
    author = "Gattringer, Christof and Lang, Christian B.",
    title = "{Quantum chromodynamics on the lattice}",
    doi = "10.1007/978-3-642-01850-3",
    isbn = "978-3-642-01849-7, 978-3-642-01850-3",
    publisher = "Springer",
    address = "Berlin",
    volume = "788",
    year = "2010"
}

@article{Luscher:1986pf,
    author = "Luscher, M.",
    title = "{Volume Dependence of the Energy Spectrum in Massive Quantum Field Theories. 2. Scattering States}",
    reportNumber = "DESY-86-034",
    doi = "10.1007/BF01211097",
    journal = "Commun. Math. Phys.",
    volume = "105",
    pages = "153--188",
    year = "1986"
}

@article{Luscher:1990ux,
    author = "Luscher, Martin",
    title = "{Two particle states on a torus and their relation to the scattering matrix}",
    reportNumber = "DESY-90-131",
    doi = "10.1016/0550-3213(91)90366-6",
    journal = "Nucl. Phys. B",
    volume = "354",
    pages = "531--578",
    year = "1991"
}

@article{Beane_2008,
   title={Multipion Systems in Lattice QCD and the Three-Pion Interaction},
   volume={100},
   ISSN={1079-7114},
   DOI={10.1103/physrevlett.100.082004},
   number={8},
   journal={Physical Review Letters},
   publisher={American Physical Society (APS)},
   author={Beane, Silas R. and Detmold, William and Luu, Thomas C. and Orginos, Kostas and Savage, Martin J. and Torok, Aaron},
   year={2008},
   month={Feb}
}

@article{Detmold:2008fn,
    author = "Detmold, William and Savage, Martin J. and Torok, Aaron and Beane, Silas R. and Luu, Thomas C. and Orginos, Kostas and Parreno, Assumpta",
    title = "{Multi-Pion States in Lattice QCD and the Charged-Pion Condensate}",
    eprint = "0803.2728",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    reportNumber = "NT@UW-08-06, LLNL-JRNL-402365, UNH-08-01, JLAB-THY-08-803",
    doi = "10.1103/PhysRevD.78.014507",
    journal = "Phys. Rev. D",
    volume = "78",
    pages = "014507",
    year = "2008"
}

@article{Mai:2018djl,
    author = "Mai, Maxim and Doring, Michael",
    title = "{Finite-Volume Spectrum of $\pi^+\pi^+$ and $\pi^+\pi^+\pi^+$ Systems}",
    eprint = "1807.04746",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    reportNumber = "JLAB-THY-18-2767",
    doi = "10.1103/PhysRevLett.122.062503",
    journal = "Phys. Rev. Lett.",
    volume = "122",
    number = "6",
    pages = "062503",
    year = "2019"
}

@article{Horz:2019rrn,
    author = {H\"orz, Ben and Hanlon, Andrew},
    title = "{Two- and three-pion finite-volume spectra at maximal isospin from lattice QCD}",
    eprint = "1905.04277",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    reportNumber = "MITP/19-033",
    doi = "10.1103/PhysRevLett.123.142002",
    journal = "Phys. Rev. Lett.",
    volume = "123",
    number = "14",
    pages = "142002",
    year = "2019"
}

@article{Culver:2019vvu,
    author = {Culver, Chris and Mai, Maxim and Brett, Ruair\'\i{} and Alexandru, Andrei and D\"oring, Michael},
    title = "{Three pion spectrum in the $I=3$ channel from lattice QCD}",
    eprint = "1911.09047",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    doi = "10.1103/PhysRevD.101.114507",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "11",
    pages = "114507",
    year = "2020"
}

@article{Blanton:2019vdk,
    author = "Blanton, Tyler D. and Romero-L\'opez, Fernando and Sharpe, Stephen R.",
    title = "{$I=3$ Three-Pion Scattering Amplitude from Lattice QCD}",
    eprint = "1909.02973",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    doi = "10.1103/PhysRevLett.124.032001",
    journal = "Phys. Rev. Lett.",
    volume = "124",
    number = "3",
    pages = "032001",
    year = "2020"
}

@article{Jackura:2020bsk,
    author = "Jackura, Andrew W. and Brice\~no, Ra\'ul A. and Dawid, Sebastian M. and Islam, Md Habib E. and McCarty, Connor",
    title = "{Solving relativistic three-body integral equations in the presence of bound states}",
    eprint = "2010.09820",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    reportNumber = "JLAB-THY-20-3272",
    doi = "10.1103/PhysRevD.104.014507",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "1",
    pages = "014507",
    year = "2021"
}

@article{Frederico:2021wej,
    author = "Frederico, T. and Ydrefors, E.",
    title = "{Three-Bosons in a Finite 4D Euclidean Volume}",
    doi = "10.1007/s00601-021-01594-4",
    journal = "Few Body Syst.",
    volume = "62",
    number = "1",
    pages = "8",
    year = "2021"
}

@article{Alexandru:2020xqf,
    author = {Alexandru, Andrei and Brett, Ruair\'\i{} and Culver, Chris and D\"oring, Michael and Guo, Dehua and Lee, Frank X. and Mai, Maxim},
    title = "{Finite-volume energy spectrum of the $K^-K^-K^-$ system}",
    eprint = "2009.12358",
    archivePrefix = "arXiv",
    primaryClass = "hep-lat",
    doi = "10.1103/PhysRevD.102.114523",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "11",
    pages = "114523",
    year = "2020"
}
@article{Thomas:1935zz,
    author = "Thomas, L. H.",
    title = "{The Interaction Between a Neutron and a Proton and the Structure of H**3}",
    doi = "10.1103/PhysRev.47.903",
    journal = "Phys. Rev.",
    volume = "47",
    pages = "903--909",
    year = "1935"
}
@article{Efimov:1970zz,
    author = "Efimov, V.",
    title = "{Energy levels arising form the resonant two-body forces in a three-body system}",
    doi = "10.1016/0370-2693(70)90349-7",
    journal = "Phys. Lett. B",
    volume = "33",
    pages = "563--564",
    year = "1970"
}
@article{Coutinho:1995zv,
    author = "Coutinho, F. A. B. and Perez, J. F. and Wreszinski, W. F.",
    title = "{A Variational proof of the Thomas effect}",
    doi = "10.1063/1.531074",
    journal = "J. Math. Phys.",
    volume = "36",
    pages = "1625--1635",
    year = "1995"
}


@article{Danilov1961,
    author = "Danilov, G. S.",
    title = "{On the three-body problem in the case of short-range forces}",
    journal = "Soviet Phys . JETP",
    volume = "13",
    pages = "349–355",
    year = "1961"
}

@article{skornyakov1956jetp,
  title={JETP 31 775 Google Scholar Skornyakov G V. and Ter-Martirosyan KA 1957},
  author={Skornyakov, GV},
  journal={Soviet Phys. JETP},
  volume={4},
  pages={648},
  year={1956}
}

@article{STM1956,
  author = {Skornyakov, G. V. and Ter-Martirosyan, K. A.},
  journal = {Sov. Phys. JETP},
  volume = {4},
  pages = {648},
  year = {1957}, 
}
